Ensuring Fairness under Prior Probability Shifts

In this paper, we study the problem of fair classification in the presence of prior probability shifts, where the training set distribution differs from the test set. This phenomenon can be observed in the yearly records of several real-world datasets, such as recidivism records and medical expenditure surveys. If unaccounted for, such shifts can cause the predictions of a classifier to become unfair towards specific population subgroups. While the fairness notion called Proportional Equality (PE) accounts for such shifts, a procedure to ensure PE-fairness was unknown. In this work, we propose a method, called CAPE, which provides a comprehensive solution to the aforementioned problem. CAPE makes novel use of prevalence estimation techniques, sampling and an ensemble of classifiers to ensure fair predictions under prior probability shifts. We introduce a metric, called prevalence difference (PD), which CAPE attempts to minimize in order to ensure PE-fairness. We theoretically establish that this metric exhibits several desirable properties. We evaluate the efficacy of CAPE via a thorough empirical evaluation on synthetic datasets. We also compare the performance of CAPE with several popular fair classifiers on real-world datasets like COMPAS (criminal risk assessment) and MEPS (medical expenditure panel survey). The results indicate that CAPE ensures PE-fair predictions, while performing well on other performance metrics.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}
%Intelligent algorithms, such as machine learning classifiers, are percolating into all aspects of modern society. Consequently, 
Classifiers are playing an increasingly crucial role in making important societal decisions, such as criminal risk assessment, hiring, sanctioning loans, etc. There is a growing concern regarding implicit discriminatory traits exhibited by classifiers' predictions towards population subgroups differentiated by race, gender, ethnicity etc. Such discrimination is unethical, and even illegal under certain circumstances~ \cite{angwin2016machine}. This has spurred research in the area of \emph{algorithmic fairness} from a wide spectrum of communities like computer science, social science, and statistics
\cite{corbett2018measure,dressel2018accuracy,chouldechova2018frontiers,friedler2018comparative,zhang2018achieving,berk2017fairness}. 
%While several earlier works have attempt to mitigate this problem, they fall short either in terms of establishing a satisfactory definition of fairness, or in terms of implementing an efficient solution which enforces fairness in the predictions. Some popular formalizations of fairness include 
Most of these papers aim at establishing fairness notions applicable for a group of individuals, and providing algorithms for ensuring fair predictions. Some popular group-fairness concepts include:

\begin{itemize}
\item \textit{Disparate Impact freeness} (DI)~\cite{feldman2015certifying,zafar2017afairness,kamiran2012data,calders2009building} and \textit{Statistical Parity} (SP)~\cite{corbett2017algorithmic,kamishima2012fairness,zemel2013learning} 
where the predictions of a classifier are said to be fair if the fraction of a population subgroup $A$ who are predicted to be in positive class, $\hat{\rho}^A$, is \textit{close} to the fraction of a population subgroup $B$ who received positive decisions, $\hat{\rho}^B$. 

\item \textit{Equalized Odds} (EO)  \cite{hardt2016equality,kleinberg2017inherent,woodworth2017learning}: The predictions on a data set satisfy \textit{equalized odds} if the false positive rate (FPR) and false negative rate (FNR) for population subgroup $A$ is \textit{close} to, respectively, the FPR and FNR for group $B$.

\item \textit{Disparate Mistreatment}  \cite{zafar2017bfairness,celis2018fairness}: The predictions on a data set are said to suffer from \textit{disparate mistreatment} if the misclassification rates differ for groups of people having different values of that sensitive attribute. One such misclassification rate is false discovery rate (FDR), which is the misclassification rate among all the positively predicted individuals from a group.

\item \textit{Proportional Equality} (PE) \cite{biswas2019fairness,crisp2014aristotle,hunter2000proportional}:  The predictions on a data set are said to be \textit{proportionally equal} if the ratio of positively predicted fraction of individuals ($\hat{\rho}^A/\hat{\rho}^B$) is close to the true ratio (${\rho}^A/{\rho}^B$). This definition considers prior probability shifts among each group.
\end{itemize}

Unfortunately, these fairness constraints turn out to be non-convex, thereby making the optimization problem---maximizing accuracy subject to fairness constraints---difficult to solve efficiently. Several papers focus on finding near-optimal near-feasible solutions~\cite{cotter2018training,celis2018classification},  or provide convex surrogates of the non-convex constraints \cite{goh2016satisfying,zafar2017afairness}, or propose pre-processing, in-processing and post-processing techniques to ensure fairness~\cite{kamiran2012data,kamiran2012decision,pleiss2017fairness,zhang2018mitigating}. 
However, most of these solutions assume that the training and test data are identically and independently drawn from some common population distribution, and thus suffer in the presence of \textit{prior probability shifts} (we observe this in our experiments). 

There are important real-world scenarios where the phenomenon known as \textit{prior probability shift} (the fraction of positively labeled instances being different in training and test datasets) occurs. As a concrete example, let us consider the COMPAS dataset~\cite{url:compas}
%is a real-world example where adhering to the static threshold of $0.8$ dictated by DI is detrimental to certain population subgroups. 
 which contains demographic information about an individual, and whether s/he recommitted a crime within a certain period of time (positive labels are given to the re-offenders, while others have negative labels). We observe that, for screening dates in the year $2013$, the fraction of re-offenders among African-American and Caucasian races were $0.486$ and $0.327$, respectively. However, in $2014$, these fractions were $0.706$ and $0.636$ respectively. Now, consider a learning problem where one uses the records of $2013$ for training, and aims to \textit{fairly} predict which defendant in $2014$ is likely to re-offend. In this example, a classifier $C$, trained to satisfy equalized odds over the $2013$ data records, may not satisfy equalized odds over the data for $2014$. We observe the same in our experimental results. %The only way $C$ can exhibit equalized odds over the data for $2014$ is if it observes the true labels, something it is barred from doing during the prediction phase.
  
One solution is to solve an optimization problem which maximizes accuracy subject to a constraint that satisfies DI ($0.8\leq\frac{\hat{\rho}^{A}}{\hat{\rho}^B}\leq 1.25$) or SP ($|{\hat{\rho}^{A}}-{\hat{\rho}^B}|\leq \epsilon$, where $\epsilon>0$ is a small number). For DI, the thresholds $0.8$ and $1.25$  are used in order to adhere to the EEOC's Uniform Guidelines\footnote{$80\%$ criterion conforms to the Uniform Guidelines on Employee Selection Procedures (August $25$, $1978$), and have been adopted by the U.S. Equal Employment Opportunity Commission, the Department of Labor, the Department of Justice, and the Civil Service Commission.} which suggest a $80\%$ criterion for curbing adverse impact in age, ethnic, race and gender discrimination cases. Unfortunately, these fairness constraints turn out to be non-convex, thereby making the optimization problem difficult to solve efficiently. Several papers focus on finding near-optimal near-feasible solutions~\cite{cotter2018training,celis2018classification},  or provide convex surrogates of the non-convex constraints \cite{goh2016satisfying,zafar2017afairness}. %However, using these convex surrogates as an optimization constraint do not necessarily ensure fairness over predictions on the test dataset, under prior-probability shifts.

Although the prior probability shift in the COMPAS data could be dealt with using the DI thresholds $0.8$ and $1.25$, however, there are other datasets, such as Medical Expenditure Panel Survey data (MEPS), where the true prevalence ratio is $2.16$. It is illogical to use $0.8$ and $1.25$ thresholds, since it would exhibit discriminatory traits for the population subgroup, or may harm both the groups. Thus, we need a more robust fairness concept which can take into account any such shifts in prior probability. Here, PE fairness notion is more appropriate, which would help the 

To the best of our knowledge, we provide the first end-to-end solution to the problem of ensuring fairness in classifiers, assuming prior probability shifts between the training and test datasets. We begin by providing a more robust notion to evaluate fairness in predictions, which we called \emph{Prevalence Difference} ($\PD$) (Section~\ref{sec:pd-fair}). Intuitively, $\PD$-fairness aims to minimize the gap between the \emph{true  prevalences} (Equation~\ref{eq:TruePrev}) and the \emph{prediction prevalences} (Equation~\ref{eq:PredPrev}), while minimally sacrificing accuracy. In Section~\ref{sec:theory}, we establish that $\PD$-fairness and accuracy are not orthogonal goals, which contrasts the impossibility result by Kleinberg et al.~\cite{kleinberg2017inherent} (no non-trivial well-calibrated classifier can satisfy EO).

We then describe our proposed solution, called $\cape$ in Section~\ref{sec:cape}. $\cape$ ensures $\PD$-fair predictions, even in the presence of prior probability shifts. It may seem that $\cape$ faces a similar hurdle as ensuring EO---ensuring $\PD$-fairness requires the knowledge of the \emph{true prevalences} of the test dataset, which in turn requires \emph{true labels} of the test dataset to be known, something which we are barred from observing while making predictions. We address this issue by \emph{estimating} the true prevalences of the test data using \emph{quantification} techniques~\cite{gonzalez2017quantification}. In Section~\ref{sec:eval}, we show empirically that the estimate obtained via quantification is a good approximation of the true prevalences, for the datasets we considered. 

$\cape$ is a combinatorial system, and does \emph{not} involve solving an optimization problem with the (non-convex) $\PD$-fairness constraint, thereby making it highly efficient, computationally. We perform a thorough experimental evaluation (in Section~\ref{sec:eval}) on synthetically generated datsets as well as real-world datasets such as COMPAS and MEPS to provide empirical evidence that $\cape$ generates $\PD$-fair predictions, while exhibiting excellent accuracy. %Surprisingly, we observe that the predictions on COMPAS dataset also exhibit $EO$.




==> tables/compas.tex <==
% & & & & \multicolumn{7}{c}{\textbf{eval ( eval)}}\\
% \cmidrule(lr){5-11}

& & \multicolumn{3}{c}{\textbf{FPR}} & \multicolumn{3}{c}{\textbf{FNR}} & \multicolumn{3}{c}{\textbf{Accuracy}} & \multicolumn{2}{c}{\begin{tabular}{@{}c@{}}\textbf{Prediction} \\ \textbf{Prevalences}\end{tabular}} & \multicolumn{2}{c}{\textbf{PD}}\\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-11}
\cmidrule(lr){12-13}
\cmidrule(lr){14-15}

& \textbf{Algorithms}
& \multicolumn{1}{c}{\textbf{Z = 0}}
& \multicolumn{1}{c}{\textbf{Z = 1}}
& \multicolumn{1}{c}{\textbf{diff}}
& \multicolumn{1}{c}{\textbf{Z = 0}}
& \multicolumn{1}{c}{\textbf{Z = 1}}
& \multicolumn{1}{c}{\textbf{diff}}
& \multicolumn{1}{c}{\textbf{Z = 0}}
& \multicolumn{1}{c}{\textbf{Z = 1}}
& \multicolumn{1}{c}{\textbf{diff}}
& \multicolumn{1}{c}{\textbf{Z = 0}}
& \multicolumn{1}{c}{\textbf{Z = 1}}
& \multicolumn{1}{c}{\textbf{Z = 0}}
& \multicolumn{1}{c}{\textbf{Z = 1}}
& \multicolumn{1}{c}{\textbf{PE}} \\[0.3em]

\toprule

\parbox[c]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\ \ $\cape$}}}
& $\cape$
& \multicolumn{1}{r}{0.461}
& \multicolumn{1}{r}{0.380}
& \multicolumn{1}{r}{0.081}
& \multicolumn{1}{r}{0.302}
& \multicolumn{1}{r}{0.275}
& \multicolumn{1}{r}{0.027}
& \multicolumn{1}{r}{0.640}
& \multicolumn{1}{r}{0.694}
& \multicolumn{1}{r}{0.054}
& \multicolumn{1}{r}{0.612}
& \multicolumn{1}{r}{0.623}
& \multicolumn{1}{r}{0.024}
& \multicolumn{1}{r}{0.083}
& \multicolumn{1}{r}{0.082}
\\

& $\cape$-1
& \multicolumn{1}{r}{0.271}
& \multicolumn{1}{r}{0.290}
& \multicolumn{1}{r}{0.019}
& \multicolumn{1}{r}{0.451}
& \multicolumn{1}{r}{0.322}
& \multicolumn{1}{r}{0.129}
& \multicolumn{1}{r}{0.614}
& \multicolumn{1}{r}{0.687}
& \multicolumn{1}{r}{0.073}
& \multicolumn{1}{r}{0.448}
& \multicolumn{1}{r}{0.564}
& \multicolumn{1}{r}{0.188}
& \multicolumn{1}{r}{0.142}
& \multicolumn{1}{r}{0.119}
\\

& $\cape$-100
& \multicolumn{1}{r}{0.488}
& \multicolumn{1}{r}{0.448}
& \multicolumn{1}{r}{0.041}
& \multicolumn{1}{r}{0.313}
& \multicolumn{1}{r}{0.263}
& \multicolumn{1}{r}{0.051}
& \multicolumn{1}{r}{0.623}
& \multicolumn{1}{r}{0.683}
& \multicolumn{1}{r}{0.060}
& \multicolumn{1}{r}{0.614}
& \multicolumn{1}{r}{0.652}
& \multicolumn{1}{r}{0.021}
& \multicolumn{1}{r}{0.054}
& \multicolumn{1}{r}{0.046}
\\[0.3em]

\midrule

%\parbox[c]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\ \ \textbf{Multithreaded}}}}
& $\BClass$
& \multicolumn{1}{r}{0.132}
& \multicolumn{1}{r}{0.259}
& \multicolumn{1}{r}{0.127}
& \multicolumn{1}{r}{0.629}
& \multicolumn{1}{r}{0.340}
& \multicolumn{1}{r}{0.289}
& \multicolumn{1}{r}{0.552}
& \multicolumn{1}{r}{0.684}
& \multicolumn{1}{r}{0.132}
& \multicolumn{1}{r}{0.284}
& \multicolumn{1}{r}{0.542}
& \multicolumn{1}{r}{0.352}
& \multicolumn{1}{r}{0.163}
& \multicolumn{1}{r}{0.376}
\\[0.3em]

\midrule 

\parbox[c]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\ \ {\textbf{Pre}}}}}

& $\mathtt{Reweigh}$
& \multicolumn{1}{r}{0.283}
& \multicolumn{1}{r}{0.139}
& \multicolumn{1}{r}{0.144}
& \multicolumn{1}{r}{0.493}
& \multicolumn{1}{r}{0.543}
& \multicolumn{1}{r}{0.050}
& \multicolumn{1}{r}{0.583}
& \multicolumn{1}{r}{0.576}
& \multicolumn{1}{r}{0.007}
& \multicolumn{1}{r}{0.425}
& \multicolumn{1}{r}{0.363}
& \multicolumn{1}{r}{0.211}
& \multicolumn{1}{r}{0.343}
& \multicolumn{1}{r}{0.271} \\ [0.4em]

\midrule

\parbox[c]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\ \ \textbf{In}}}}
& $\mathtt{Meta}$-$\mathtt{fair}$-sr
& \multicolumn{1}{r}{0.977}
& \multicolumn{1}{r}{0.849}
& \multicolumn{1}{r}{0.128}
& \multicolumn{1}{r}{0.102}
& \multicolumn{1}{r}{0.492}
& \multicolumn{1}{r}{0.390}
& \multicolumn{1}{r}{0.579}
& \multicolumn{1}{r}{0.403}
& \multicolumn{1}{r}{0.176}
& \multicolumn{1}{r}{0.927}
& \multicolumn{1}{r}{0.609}
& \multicolumn{1}{r}{0.291}
& \multicolumn{1}{r}{0.097}
& \multicolumn{1}{r}{0.622}
\\

& $\mathtt{Meta}$-$\mathtt{fair}$-fdr
& \multicolumn{1}{r}{0.965}
& \multicolumn{1}{r}{0.901}
& \multicolumn{1}{r}{0.064}
& \multicolumn{1}{r}{0.162}
& \multicolumn{1}{r}{0.356}
& \multicolumn{1}{r}{0.194}
& \multicolumn{1}{r}{0.545}
& \multicolumn{1}{r}{0.483}
& \multicolumn{1}{r}{0.062}
& \multicolumn{1}{r}{0.884}
& \multicolumn{1}{r}{0.719}
& \multicolumn{1}{r}{0.248}
& \multicolumn{1}{r}{0.013}
& \multicolumn{1}{r}{0.329}
\\

& $\mathtt{AD}$
& \multicolumn{1}{r}{0.124}
& \multicolumn{1}{r}{0.167}
& \multicolumn{1}{r}{0.043}
& \multicolumn{1}{r}{0.638}
& \multicolumn{1}{r}{0.467}
& \multicolumn{1}{r}{0.171}
& \multicolumn{1}{r}{0.549}
& \multicolumn{1}{r}{0.621}
& \multicolumn{1}{r}{0.072}
& \multicolumn{1}{r}{0.275}
& \multicolumn{1}{r}{0.425}
& \multicolumn{1}{r}{0.361}
& \multicolumn{1}{r}{0.281}
& \multicolumn{1}{r}{0.253}
\\
[0.3em]

\midrule 

\parbox[c]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\ \ \textbf{Post}}}}
& $\mathtt{CEOP}$-fpr
& \multicolumn{1}{r}{0.066}
& \multicolumn{1}{r}{1.000}
& \multicolumn{1}{r}{0.934}
& \multicolumn{1}{r}{0.722}
& \multicolumn{1}{r}{0.000}
& \multicolumn{1}{r}{0.722}
& \multicolumn{1}{r}{0.517}
& \multicolumn{1}{r}{0.706}
& \multicolumn{1}{r}{0.189}
& \multicolumn{1}{r}{0.201}
& \multicolumn{1}{r}{1.000}
& \multicolumn{1}{r}{0.435}
& \multicolumn{1}{r}{0.294}
& \multicolumn{1}{r}{0.699}
\\

& $\mathtt{CEOP}$-fnr
& \multicolumn{1}{r}{0.000}
& \multicolumn{1}{r}{0.247}
& \multicolumn{1}{r}{0.247}
& \multicolumn{1}{r}{1.000}
& \multicolumn{1}{r}{0.390}
& \multicolumn{1}{r}{0.610}
& \multicolumn{1}{r}{0.364}
& \multicolumn{1}{r}{0.652}
& \multicolumn{1}{r}{0.288}
& \multicolumn{1}{r}{0.000}
& \multicolumn{1}{r}{0.503}
& \multicolumn{1}{r}{0.636}
& \multicolumn{1}{r}{0.203}
& \multicolumn{1}{r}{0.900}
\\

& $\mathtt{CEOP}$-weighted
& \multicolumn{1}{r}{0.000}
& \multicolumn{1}{r}{0.194}
& \multicolumn{1}{r}{0.194}
& \multicolumn{1}{r}{1.000}
& \multicolumn{1}{r}{0.405}
& \multicolumn{1}{r}{0.495}
& \multicolumn{1}{r}{0.364}
& \multicolumn{1}{r}{0.657}
& \multicolumn{1}{r}{0.292}
& \multicolumn{1}{r}{0.000}
& \multicolumn{1}{r}{0.477}
& \multicolumn{1}{r}{0.636}
& \multicolumn{1}{r}{0.229}
& \multicolumn{1}{r}{0.900}
\\

& $\mathtt{ROC}$-spd
& \multicolumn{1}{r}{0.919}
& \multicolumn{1}{r}{0.994}
& \multicolumn{1}{r}{0.075}
& \multicolumn{1}{r}{0.031}
& \multicolumn{1}{r}{0.004}
& \multicolumn{1}{r}{0.027}
& \multicolumn{1}{r}{0.645}
& \multicolumn{1}{r}{0.705}
& \multicolumn{1}{r}{0.060}
& \multicolumn{1}{r}{0.951}
& \multicolumn{1}{r}{0.995}
& \multicolumn{1}{r}{0.315}
& \multicolumn{1}{r}{0.289}
& \multicolumn{1}{r}{0.056}
\\

& $\mathtt{ROC}$-aod
& \multicolumn{1}{r}{0.004}
& \multicolumn{1}{r}{0.019}
& \multicolumn{1}{r}{0.015}
& \multicolumn{1}{r}{0.978}
& \multicolumn{1}{r}{0.900}
& \multicolumn{1}{r}{0.078}
& \multicolumn{1}{r}{0.377}
& \multicolumn{1}{r}{0.360}
& \multicolumn{1}{r}{0.017}
& \multicolumn{1}{r}{0.016}
& \multicolumn{1}{r}{0.076}
& \multicolumn{1}{r}{0.620}
& \multicolumn{1}{r}{0.630}
& \multicolumn{1}{r}{0.879}
\\

& $\mathtt{ROC}$-eod
& \multicolumn{1}{r}{0.019}
& \multicolumn{1}{r}{0.046}
& \multicolumn{1}{r}{0.027}
& \multicolumn{1}{r}{0.911}
& \multicolumn{1}{r}{0.782}
& \multicolumn{1}{r}{0.129}
& \multicolumn{1}{r}{0.414}
& \multicolumn{1}{r}{0.434}
& \multicolumn{1}{r}{0.020}
& \multicolumn{1}{r}{0.064}
& \multicolumn{1}{r}{0.167}
& \multicolumn{1}{r}{0.572}
& \multicolumn{1}{r}{0.539}
& \multicolumn{1}{r}{0.517}
\\

\bottomrule


==> tables/meps.tex <==
% & & & & \multicolumn{7}{c}{\textbf{eval ( eval)}}\\
% \cmidrule(lr){5-11}

& & \multicolumn{3}{c}{\textbf{FPR}} & \multicolumn{3}{c}{\textbf{FNR}} & \multicolumn{3}{c}{\textbf{Accuracy}} & \multicolumn{2}{c}{\begin{tabular}{@{}c@{}}\textbf{Prediction} \\ \textbf{Prevalences}\end{tabular}} & \multicolumn{2}{c}{\textbf{PD}}\\
    \cmidrule(lr){3-5}
    \cmidrule(lr){6-8}
    \cmidrule(lr){9-11}
    \cmidrule(lr){12-13}
    \cmidrule(lr){14-15}
    
    & \textbf{Algorithms}
    & \multicolumn{1}{c}{\textbf{Z = 0}}
    & \multicolumn{1}{c}{\textbf{Z = 1}}
    & \multicolumn{1}{c}{\textbf{diff}}
    & \multicolumn{1}{c}{\textbf{Z = 0}}
    & \multicolumn{1}{c}{\textbf{Z = 1}}
    & \multicolumn{1}{c}{\textbf{diff}}
    & \multicolumn{1}{c}{\textbf{Z = 0}}
    & \multicolumn{1}{c}{\textbf{Z = 1}}
    & \multicolumn{1}{c}{\textbf{diff}}
    & \multicolumn{1}{c}{\textbf{Z = 0}}
    & \multicolumn{1}{c}{\textbf{Z = 1}}
    & \multicolumn{1}{c}{\textbf{Z = 0}}
    & \multicolumn{1}{c}{\textbf{Z = 1}}
    & \multicolumn{1}{c}{\textbf{PE}} \\[0.3em]
    
    \toprule
    \parbox[c]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\ \ $\cape$}}}
    & $\cape$
    & \multicolumn{1}{r}{0.131}
    & \multicolumn{1}{r}{0.068}
    & \multicolumn{1}{r}{0.063}
    & \multicolumn{1}{r}{0.425}
    & \multicolumn{1}{r}{0.488}
    & \multicolumn{1}{r}{0.063}
    & \multicolumn{1}{r}{0.794}
    & \multicolumn{1}{r}{0.883}
    & \multicolumn{1}{r}{0.089}
    & \multicolumn{1}{r}{0.243}
    & \multicolumn{1}{r}{0.120}
    & \multicolumn{1}{r}{0.010}
    & \multicolumn{1}{r}{0.003}
    & \multicolumn{1}{r}{0.135}
    \\

    & $\cape$-1
    & \multicolumn{1}{r}{0.175}
    & \multicolumn{1}{r}{0.087}
    & \multicolumn{1}{r}{0.088}
    & \multicolumn{1}{r}{0.347}
    & \multicolumn{1}{r}{0.423}
    & \multicolumn{1}{r}{0.076}
    & \multicolumn{1}{r}{0.781}
    & \multicolumn{1}{r}{0.874}
    & \multicolumn{1}{r}{0.093}
    & \multicolumn{1}{r}{0.296}
    & \multicolumn{1}{r}{0.144}
    & \multicolumn{1}{r}{0.043}
    & \multicolumn{1}{r}{0.027}
    & \multicolumn{1}{r}{0.049}
    \\

    & $\cape$-100
    & \multicolumn{1}{r}{0.131}
    & \multicolumn{1}{r}{0.068}
    & \multicolumn{1}{r}{0.063}
    & \multicolumn{1}{r}{0.425}
    & \multicolumn{1}{r}{0.488}
    & \multicolumn{1}{r}{0.063}
    & \multicolumn{1}{r}{0.794}
    & \multicolumn{1}{r}{0.883}
    & \multicolumn{1}{r}{0.089}
    & \multicolumn{1}{r}{0.243}
    & \multicolumn{1}{r}{0.120}
    & \multicolumn{1}{r}{0.010}
    & \multicolumn{1}{r}{0.003}
    & \multicolumn{1}{r}{0.135}
    \\[0.3em]
    
    \midrule
    
    %\parbox[c]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\ \ \textbf{Multithreaded}}}}
    & $\BClass$
    & \multicolumn{1}{r}{0.004}
    & \multicolumn{1}{r}{0.012}
    & \multicolumn{1}{r}{0.008}
    & \multicolumn{1}{r}{0.910}
    & \multicolumn{1}{r}{0.888}
    & \multicolumn{1}{r}{0.022}
    & \multicolumn{1}{r}{0.766}
    & \multicolumn{1}{r}{0.890}
    & \multicolumn{1}{r}{0.124}
    & \multicolumn{1}{r}{0.037}
    & \multicolumn{1}{r}{0.014}
    & \multicolumn{1}{r}{0.216}
    & \multicolumn{1}{r}{0.103}
    & \multicolumn{1}{r}{0.483}
    \\[0.3em]
    
    \midrule 
  
    \parbox[c]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\ \ {\textbf{Pre}}}}}
    
    & $\mathtt{Reweigh}$
    & \multicolumn{1}{r}{0.276}
    & \multicolumn{1}{r}{0.242}
    & \multicolumn{1}{r}{0.034}
    & \multicolumn{1}{r}{0.250}
    & \multicolumn{1}{r}{0.226}
    & \multicolumn{1}{r}{0.024}
    & \multicolumn{1}{r}{0.731}
    & \multicolumn{1}{r}{0.760}
    & \multicolumn{1}{r}{0.029}
    & \multicolumn{1}{r}{0.396}
    & \multicolumn{1}{r}{0.305}
    & \multicolumn{1}{r}{0.143}
    & \multicolumn{1}{r}{0.188}
    & \multicolumn{1}{r}{0.862} \\ [0.4em]
    
    \midrule 

    \parbox[c]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\ \ \textbf{In}}}}
    & $\mathtt{Meta}$-$\mathtt{fair}$-sr
    & \multicolumn{1}{r}{0.322}
    & \multicolumn{1}{r}{0.213}
    & \multicolumn{1}{r}{0.109}
    & \multicolumn{1}{r}{0.210}
    & \multicolumn{1}{r}{0.243}
    & \multicolumn{1}{r}{0.033}
    & \multicolumn{1}{r}{0.706}
    & \multicolumn{1}{r}{0.783}
    & \multicolumn{1}{r}{0.077}
    & \multicolumn{1}{r}{0.440}
    & \multicolumn{1}{r}{0.277}
    & \multicolumn{1}{r}{0.187}
    & \multicolumn{1}{r}{0.160}
    & \multicolumn{1}{r}{0.572}
    \\
    
    & $\mathtt{Meta}$-$\mathtt{fair}$-fdr
    & \multicolumn{1}{r}{0.347}
    & \multicolumn{1}{r}{0.254}
    & \multicolumn{1}{r}{0.102}
    & \multicolumn{1}{r}{0.193}
    & \multicolumn{1}{r}{0.218}
    & \multicolumn{1}{r}{0.025}
    & \multicolumn{1}{r}{0.692}
    & \multicolumn{1}{r}{0.758}
    & \multicolumn{1}{r}{0.066}
    & \multicolumn{1}{r}{0.463}
    & \multicolumn{1}{r}{0.308}
    & \multicolumn{1}{r}{0.210}
    & \multicolumn{1}{r}{0.191}
    & \multicolumn{1}{r}{0.657}
    \\
    
    & $\mathtt{AD}$
    & \multicolumn{1}{r}{0.062}
    & \multicolumn{1}{r}{0.051}
    & \multicolumn{1}{r}{0.011}
    & \multicolumn{1}{r}{0.644}
    & \multicolumn{1}{r}{0.569}
    & \multicolumn{1}{r}{0.075}
    & \multicolumn{1}{r}{0.791}
    & \multicolumn{1}{r}{0.889}
    & \multicolumn{1}{r}{0.098}
    & \multicolumn{1}{r}{0.136}
    & \multicolumn{1}{r}{0.095}
    & \multicolumn{1}{r}{0.117}
    & \multicolumn{1}{r}{0.022}
    & \multicolumn{1}{r}{0.728}
    \\
    [0.3em]
    
    \midrule 
    
    \parbox[c]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\ \ \textbf{Post}}}}
    & $\mathtt{CEOP}$-fpr
    & \multicolumn{1}{r}{0.078}
    & \multicolumn{1}{r}{0.000}
    & \multicolumn{1}{r}{0.078}
    & \multicolumn{1}{r}{0.573}
    & \multicolumn{1}{r}{1.000}
    & \multicolumn{1}{r}{0.427}
    & \multicolumn{1}{r}{0.797}
    & \multicolumn{1}{r}{0.883}
    & \multicolumn{1}{r}{0.086}
    & \multicolumn{1}{r}{0.166}
    & \multicolumn{1}{r}{0.000}
    & \multicolumn{1}{r}{0.087}
    & \multicolumn{1}{r}{0.117}
    & \multicolumn{1}{r}{$\mathtt{undef}$}
    \\
    
    & $\mathtt{CEOP}$-fnr
    & \multicolumn{1}{r}{0.034}
    & \multicolumn{1}{r}{0.022}
    & \multicolumn{1}{r}{0.012}
    & \multicolumn{1}{r}{0.803}
    & \multicolumn{1}{r}{0.704}
    & \multicolumn{1}{r}{0.102}
    & \multicolumn{1}{r}{0.771}
    & \multicolumn{1}{r}{0.899}
    & \multicolumn{1}{r}{0.128}
    & \multicolumn{1}{r}{0.075}
    & \multicolumn{1}{r}{0.054}
    & \multicolumn{1}{r}{0.178}
    & \multicolumn{1}{r}{0.063}
    & \multicolumn{1}{r}{0.771}
    \\
    
    & $\mathtt{CEOP}$-weighted
    & \multicolumn{1}{r}{0.032}
    & \multicolumn{1}{r}{0.021}
    & \multicolumn{1}{r}{0.011}
    & \multicolumn{1}{r}{0.816}
    & \multicolumn{1}{r}{0.704}
    & \multicolumn{1}{r}{0.112}
    & \multicolumn{1}{r}{0.770}
    & \multicolumn{1}{r}{0.899}
    & \multicolumn{1}{r}{0.129}
    & \multicolumn{1}{r}{0.070}
    & \multicolumn{1}{r}{0.053}
    & \multicolumn{1}{r}{0.183}
    & \multicolumn{1}{r}{0.064}
    & \multicolumn{1}{r}{0.839}
    \\
    
    & $\mathtt{ROC}$-spd
    & \multicolumn{1}{r}{0.233}
    & \multicolumn{1}{r}{0.220}
    & \multicolumn{1}{r}{0.013}
    & \multicolumn{1}{r}{0.284}
    & \multicolumn{1}{r}{0.243}
    & \multicolumn{1}{r}{0.041}
    & \multicolumn{1}{r}{0.754}
    & \multicolumn{1}{r}{0.777}
    & \multicolumn{1}{r}{0.023}
    & \multicolumn{1}{r}{0.355}
    & \multicolumn{1}{r}{0.283}
    & \multicolumn{1}{r}{0.102}
    & \multicolumn{1}{r}{0.166}
    & \multicolumn{1}{r}{0.906}
    \\
    
    & $\mathtt{ROC}$-aod
    & \multicolumn{1}{r}{0.329}
    & \multicolumn{1}{r}{0.253}
    & \multicolumn{1}{r}{0.076}
    & \multicolumn{1}{r}{0.205}
    & \multicolumn{1}{r}{0.210}
    & \multicolumn{1}{r}{0.005}
    & \multicolumn{1}{r}{0.702}
    & \multicolumn{1}{r}{0.752}
    & \multicolumn{1}{r}{0.050}
    & \multicolumn{1}{r}{0.447}
    & \multicolumn{1}{r}{0.216}
    & \multicolumn{1}{r}{0.194}
    & \multicolumn{1}{r}{0.199}
    & \multicolumn{1}{r}{0.745}
    \\
    
    & $\mathtt{ROC}$-eod
    & \multicolumn{1}{r}{0.336}
    & \multicolumn{1}{r}{0.233}
    & \multicolumn{1}{r}{0.103}
    & \multicolumn{1}{r}{0.194}
    & \multicolumn{1}{r}{0.227}
    & \multicolumn{1}{r}{0.033}
    & \multicolumn{1}{r}{0.700}
    & \multicolumn{1}{r}{0.768}
    & \multicolumn{1}{r}{0.068}
    & \multicolumn{1}{r}{0.455}
    & \multicolumn{1}{r}{0.296}
    & \multicolumn{1}{r}{0.202}
    & \multicolumn{1}{r}{0.179}
    & \multicolumn{1}{r}{0.623}
    \\
    
    \bottomrule
    

==> tables/oldTables.tex <==
\begin{table*}[!ht]
\small
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\cline{1-2} \cline{4-12}
\multicolumn{2}{|c|}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}COMPAS\\ dataset\\ $\ $\end{tabular}}}} & \multirow{2}{*}{} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Training Data}\\ \textbf{True Prevalence}\\ ${\rho_{D}^z}$\\ \\ $\ $\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Test Data}\\ \textbf{True Prevalence}\\ ${\rho_{\Testdata}^z}$\\ \\ $\ $\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Quantifier's}\\ \textbf{Estimate}\\ ${\hat{q}^z(\Testdata^z)}$\\ \\ $\ $\end{tabular}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Prediction \\ Prevalence\end{tabular}}} & \multicolumn{2}{c|}{\textbf{PD-Fair}} & \multicolumn{2}{c|}{\textbf{Accuracy}} \\ \cline{7-12} 
\multicolumn{2}{|c|}{} &  &  &  &  & \multirow{2}{*}{$\mathbf{\cape}$} & \multirow{2}{*}{$\mathbf{\BClass}$} & \multirow{2}{*}{$\mathbf{\cape}$} & \multirow{2}{*}{$\mathbf{\BClass}$} & \multirow{2}{*}{$\mathbf{\cape}$} & \multirow{2}{*}{$\mathbf{\BClass}$} \\
\multicolumn{2}{|c|}{} &  &  &  &  &  &  &  &  &  &  \\ \hline
\multicolumn{2}{|c|}{$\mathbf{z=0}$} & \multirow{2}{*}{} & $0.327$ & $0.636$ & $0.592$ & \multicolumn{1}{r|}{$0.647$} & \multicolumn{1}{r|}{$0.284$} & \cmark & \xmark & \multicolumn{1}{r|}{$0.641$} & \multicolumn{1}{r|}{$0.552$} \\ \cline{1-2} \cline{4-12} 
\multicolumn{2}{|c|}{$\mathbf{z=1}$} &  & $0.486$ & $0.706$ & $0.644$ & \multicolumn{1}{r|}{$0.649$} & \multicolumn{1}{r|}{$0.542$} & \cmark & \xmark & \multicolumn{1}{r|}{$0.687$} & \multicolumn{1}{r|}{$0.684$} \\ \hline
\end{tabular}
\caption{The COMPAS records are split into train and test based on their year of screening. The prior probability shift phenomenon is observed in columns $2$ and $3$. We observe that the quantifier generates good estimates of the true prevalences of the test dataset. Moreover, $\Delta_{\Testdata}^{z}$ for $\cape$ is always less than $0.06$, making it $\PD$-fair, while $\Delta_{\Testdata}^{0}$ for $\BClass$ is as high as $0.352$ and is thus unfair. We also note that the accuracy of $\cape$ is higher than $\BClass$, for $z \in \{0,1\}$. \label{table:compas_results}}
\end{table*}

\begin{table}[h!]
\begin{tabular}{|l|l|l|c|c|r|r|c|c|r|r|}
\cline{1-2} \cline{4-11}
\multicolumn{2}{|c|}{\multirow{3}{*}{\textbf{Dataset}}} & \multirow{2}{*}{} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{True}\\ \textbf{Prevalence}\\ ${\rho_{\Testdata}^z}$\\ \\ $\ $\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Quantifier's}\\ \textbf{Estimate}\\ ${\hat{q}^z(\Testdata^z)}$\\ \\ $\ $\end{tabular}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Prediction \\ Prevalence\end{tabular}}} & \multicolumn{2}{c|}{\textbf{PD-Fair}} & \multicolumn{2}{c|}{\textbf{Accuracy}} \\ \cline{6-11} 
\multicolumn{2}{|c|}{} &  &  &  & \multicolumn{1}{c|}{\multirow{2}{*}{$\mathbf{\cape}$}} & \multicolumn{1}{c|}{\multirow{2}{*}{$\mathbf{\BClass}$}} & \multirow{2}{*}{$\mathbf{\cape}$} & \multirow{2}{*}{$\mathbf{\BClass}$} & \multicolumn{1}{c|}{\multirow{2}{*}{$\mathbf{\cape}$}} & \multicolumn{1}{c|}{\multirow{2}{*}{$\mathbf{\BClass}$}} \\
\multicolumn{2}{|c|}{} &  &  &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\ \hline
\multirow{2}{*}{German Credit} & $\mathbf{z=0}$ & \multirow{2}{*}{} & $0.272$ & $0.288$ & $0.292$ & $0.177$ & \cmark & \xmark & $0.730$ & $0.763$ \\ \cline{2-2} \cline{4-11} 
 & $\mathbf{z=1}$ &  & $0.339$ & $0.394$ & $0.391$ & $0.259$ & \cmark & \xmark & $0.704$ & $0.745$ \\ \hline
\multirow{2}{*}{Adult Income} & $\mathbf{z=0}$ & \multirow{2}{*}{} & $0.315$ & $0.269$ & $0.285$ & $0.200$ & \cmark & \xmark & $0.805$ & $0.807$ \\ \cline{2-2} \cline{4-11} 
 & $\mathbf{z=1}$ &  & $0.115$ & $0.078$ & $0.085$ & $0.035$ & \cmark & \xmark & $0.910$ & $0.912$ \\ \hline
\end{tabular}
\caption{\label{table:other_results} Summary of fairness and accuracy results, averaged over $20$ iterations, for German Credit and Adult Income datasets. Column $3$ shows that the $\qalgo$ module of $\cape$ provides a good estimate of the true prevalences. The next two columns contain the prediction prevalences of $\cape$ and $\BClass$. For both the datasets, $\Delta^z_{\Testdata} < 0.06$ for $\cape$, making it $\PD$-fair. The $\Delta^z_{\Testdata}$ values for $\BClass$ always exceed $0.06$, making it unfair for both datasets. Though $\BClass$ performs better than $\cape$ in terms of accuracy, the absolute difference between the two is at most $0.041$, across both datasets.}  
\end{table}

==> tables/quant-compas.tex <==
% & & & & \multicolumn{7}{c}{\textbf{eval ( eval)}}\\
% \cmidrule(lr){5-11}

\textbf{\begin{tabular}[c]{@{}c@{}}$\ $\\ $ $\\ \textbf{Z} \\ \ \end{tabular}}
&  \textbf{\begin{tabular}[c]{@{}c@{}}Training Data\\ True Prevalence\\ ${\rho_{D}^z}$ \\ \ \end{tabular}}
& \textbf{\begin{tabular}[c]{@{}c@{}}Test Data\\ True Prevalence\\ ${\rho_{\Testdata}^z}$ \\ \ \end{tabular}}
& \textbf{\begin{tabular}[c]{@{}c@{}}Quantifier's\\ Estimate\\ ${\hat{q}^z(\Testdata^z)}$ \\ \ \end{tabular}} \\
\toprule
\multicolumn{1}{c}{\textbf{0}}
& \multicolumn{1}{c}{0.327}
& \multicolumn{1}{c}{0.636}
& \multicolumn{1}{c}{0.592}

\\[0.3em]

\multicolumn{1}{c}{\textbf{1}}
& \multicolumn{1}{c}{0.486}
& \multicolumn{1}{c}{0.706}
& \multicolumn{1}{c}{0.644}

\\[0.3em]

\bottomrule


==> tables/quant-meps.tex <==
% & & & & \multicolumn{7}{c}{\textbf{eval ( eval)}}\\
% \cmidrule(lr){5-11}

\textbf{\begin{tabular}[c]{@{}c@{}}$\ $\\ $\ $\\ \textbf{Z} \\ \end{tabular}}
&  \textbf{\begin{tabular}[c]{@{}c@{}}Training Data\\ True Prevalence\\ ${\rho_{D}^z}$ \\ \end{tabular}}
& \textbf{\begin{tabular}[c]{@{}c@{}}Test Data\\ True Prevalence\\ ${\rho_{\Testdata}^z}$ \\ \end{tabular}}
& \textbf{\begin{tabular}[c]{@{}c@{}}Quantifier's\\ Estimate\\ ${\hat{q}^z(\Testdata^z)}$ \\ \end{tabular}} \\

\toprule

\multicolumn{1}{c}{\textbf{0}}
& \multicolumn{1}{c}{0.253}
& \multicolumn{1}{c}{0.253}
& \multicolumn{1}{c}{0.273}

\\[0.3em]

\multicolumn{1}{c}{\textbf{1}}
& \multicolumn{1}{c}{0.124}
& \multicolumn{1}{c}{0.117}
& \multicolumn{1}{c}{0.123}

\\[0.3em]

\bottomrule

